Optimal DR-Submodular Maximization and Applications to Provable Mean Field Inference

Mean field inference in probabilistic models is generally a highly nonconvex problem. Existing optimization methods, e.g., coordinate ascent algorithms, can only generate local optima. In this work we propose provable mean filed methods for probabilistic log-submodular models and its posterior agreement (PA) with strong approximation guarantees. The main algorithmic technique is a new Double Greedy scheme, termed DR-DoubleGreedy, for continuous DR-submodular maximization with box-constraints. It is a one-pass algorithm with linear time complexity, reaching the optimal 1/2 approximation ratio, which may be of independent interest. We validate the superior performance of our algorithms against baseline algorithms on both synthetic and real-world datasets.

==> bigtable.tex <==

{
	\begin{table}
		\begin{center}
		\footnotesize
			\caption{Summary of results on ELBO objective \labelcref{opt_problem_meanfield} and PA-ELBO objective \labelcref{pa_elbo}. \algname{Sub-DG} stands for  \algname{Submodular-DoubleGreedy}, \algname{DR-DG} stands for  \algname{DR-DoubleGreedy}. Boldface numbers indicate the best mean of function values returned. For ELBO,  the mean and standard deviation were calculated
				for 10 FLID models trained on 10 folds of the data. For PA-ELBO, the mean and standard deviation were calculated  for models trained over $45$ pairs of folds. More details are in the experimental section.}
			\label{tab_summ_elbo}
			\begin{tabular}{|c|c||c|c|c||c|c|c|}
				\cline{1-8} 
				&  &  \multicolumn{3}{|c||}{\textbf{ELBO} objective \labelcref{opt_problem_meanfield}} &  \multicolumn{3}{|c|}{\textbf{PA-ELBO} objective \labelcref{pa_elbo}}  \\
				\cline{1-8}
				Category	& $D$ &  \algname{Sub-DG} & \algname{BSCB} & \algname{DR-DG} &  \algname{Sub-DG} & \algname{BSCB} & \algname{DR-DG} \\
				\hline
				\hline
				\multirow{2}{*}{furniture}  & 2  & 2.078$\pm$0.091 & 2.771$\pm$0.123  & \textbf{3.035}$\pm$0.059  & 0.918$\pm$0.768 & 2.287$\pm$0.399  & \textbf{2.402}$\pm$0.159\\
				%\cline{2-5}
				& 3  & 1.835$\pm$0.156 & 2.842$\pm$0.128  & \textbf{3.026}$\pm$0.099 & 1.296$\pm$1.176 & 2.536$\pm$0.439  & \textbf{2.693}$\pm$0.181 \\
				%\cline{2-5}
				$n$=32 & 10  & 1.375$\pm$0.194 & \textbf{2.951}$\pm$0.161  & {2.917}$\pm$0.103 & 1.504$\pm$1.110 & 2.764$\pm$0.405  & \textbf{2.882}$\pm$0.248 \\
				\hline
				\multirow{2}{*}{carseats}  & 2  & 2.089$\pm$0.166 & 2.863$\pm$0.090  & \textbf{3.045}$\pm$0.069 & 1.015$\pm$1.081 & 2.106$\pm$0.228  & \textbf{2.348}$\pm$0.219\\
				%\cline{2-5}
				& 3  & 1.890$\pm$0.146 & 3.003$\pm$0.110  & \textbf{3.138}$\pm$0.082 & 1.309$\pm$1.218 & 2.414$\pm$0.267  & \textbf{2.707}$\pm$0.208 \\
				%\cline{2-5}
				$n$=34 & 10  & 1.390$\pm$0.232 & \textbf{3.100}$\pm$0.140  & {3.003}$\pm$0.157 & 1.599$\pm$1.317 & 2.684$\pm$0.271  & \textbf{2.915}$\pm$0.250 \\
				\hline
				\multirow{2}{*}{safety}  & 2  & 1.934$\pm$0.402 & 2.727$\pm$0.212  & \textbf{2.896}$\pm$0.098 & 1.370$\pm$1.203 & 2.049$\pm$0.280  & \textbf{2.341}$\pm$0.161\\
				%\cline{2-5}
				& 3  & 1.867$\pm$0.453 & 2.830$\pm$0.191  & \textbf{2.970}$\pm$0.110 & 1.706$\pm$1.296 & 2.288$\pm$0.297  & \textbf{2.619}$\pm$0.167 \\
				%\cline{2-5}
				$n$=36 & 10  & 1.546$\pm$0.606 & 2.916$\pm$0.191  & \textbf{2.920}$\pm$0.149 & 1.948$\pm$1.353 & 2.467$\pm$0.270  & \textbf{2.738}$\pm$0.187 \\
				\hline
				\multirow{2}{*}{strollers}  & 2  & 2.042$\pm$0.181 & 2.829$\pm$0.144  & \textbf{2.928}$\pm$0.060 & 0.865$\pm$0.952 & 1.933$\pm$0.256  & \textbf{2.202}$\pm$0.226\\
				%\cline{2-5}
				& 3  & 1.814$\pm$0.264 & 2.958$\pm$0.146  & \textbf{2.978}$\pm$0.077 & 1.172$\pm$1.063 & 2.181$\pm$0.297  & \textbf{2.543}$\pm$0.254 \\
				%\cline{2-5}
				$n$=40 & 10  & 1.328$\pm$0.544 & \textbf{3.065}$\pm$0.162  & 2.910$\pm$0.140 & 1.702$\pm$1.334 & 2.480$\pm$0.304  & \textbf{2.767}$\pm$0.336 \\
				\hline
				\multirow{2}{*}{media}  & 2  & 3.221$\pm$0.066 & 3.309$\pm$0.055  & \textbf{3.493}$\pm$0.051 & 0.372$\pm$0.286 &\textbf{ 1.477}$\pm$0.128  & 1.336$\pm$0.101\\
%				\cline{2-5}
				& 3  & 3.276$\pm$0.082 & 3.492$\pm$0.083  & \textbf{3.712}$\pm$0.079 & 0.418$\pm$0.366 & 1.736$\pm$0.177  & \textbf{1.762}$\pm$0.095 \\
%				\cline{2-5}
				$n$=58 & 10  & 2.840$\pm$0.183 & 3.894$\pm$0.122  & \textbf{3.924}$\pm$0.114 & 0.653$\pm$0.727 & 2.309$\pm$0.244  & \textbf{2.524}$\pm$0.130 \\
				\hline
				\multirow{2}{*}{health}  & 2  & 3.197$\pm$0.067 & 3.174$\pm$0.074  & \textbf{3.516}$\pm$0.043 & 0.548$\pm$0.282 & \textbf{1.655}$\pm$0.122  & 1.650$\pm$0.073\\
				%\cline{2-5}
				& 3  & 3.231$\pm$0.055 & 3.306$\pm$0.108  & \textbf{3.707}$\pm$0.064 & 0.649$\pm$0.413 & 1.903$\pm$0.173  & \textbf{2.025}$\pm$0.083 \\
				%\cline{2-5}
				$n$=62 & 10  & 2.633$\pm$0.115 & 3.508$\pm$0.120  & \textbf{3.675}$\pm$0.110 & 0.768$\pm$0.628 & 2.233$\pm$0.196  & \textbf{2.375}$\pm$0.101 \\
				\hline
				\multirow{2}{*}{toys}  & 2  & 3.543$\pm$0.047 & 3.454$\pm$0.091  & \textbf{3.856}$\pm$0.044 & 0.597$\pm$0.480 & 1.731$\pm$0.182  & \textbf{{1.761}}$\pm$0.133\\
				%\cline{2-5}
				& 3  & 3.362$\pm$0.055 & 3.412$\pm$0.070  & \textbf{3.736}$\pm$0.051 & 0.578$\pm$0.520 & 1.738$\pm$0.192  & \textbf{1.802}$\pm$0.151 \\
				%\cline{2-5}
				$n$=62 & 10  & 3.037$\pm$0.138 & 3.706$\pm$0.108  & \textbf{3.859}$\pm$0.119 & 0.758$\pm$0.871 & 2.140$\pm$0.242  & \textbf{2.330}$\pm$0.177 \\
				\hline
				\multirow{2}{*}{diaper}  & 2  & 3.500$\pm$0.058 & 3.517$\pm$0.058  & \textbf{3.636}$\pm$0.043 & 0.295$\pm$0.158 & \textbf{1.119}$\pm$0.063  & 0.665$\pm$0.116\\
				%\cline{2-5}
				& 3  & 3.739$\pm$0.080 & 3.753$\pm$0.065  & \textbf{3.974}$\pm$0.065 & 0.337$\pm$0.240 & \textbf{1.429}$\pm$0.111  & 1.141$\pm$0.120 \\
				%\cline{2-5}
				$n$=100 & 10  & 3.423$\pm$0.110 & 4.150$\pm$0.120  & \textbf{4.203}$\pm$0.086 & 0.386$\pm$0.504 & 1.969$\pm$0.201  & \textbf{2.009}$\pm$0.199 \\
				\hline
				\multirow{2}{*}{feeding}  & 2  & 3.942$\pm$0.041 & 3.808$\pm$0.024  & \textbf{3.970}$\pm$0.036 & 0.393$\pm$0.034 & \textbf{0.894}$\pm$0.022  & 0.501$\pm$0.029\\
%				\cline{2-5}
				& 3  & 4.333$\pm$0.031 & 4.095$\pm$0.032  & \textbf{4.390}$\pm$0.031 & 0.503$\pm$0.072 & \textbf{1.232}$\pm$0.041  & 0.893$\pm$0.046 \\
				%\cline{2-5}
				$n$=100 & 10  & 4.611$\pm$0.053 & 4.553$\pm$0.079  & \textbf{4.860}$\pm$0.056 & 0.608$\pm$0.239 & 1.808$\pm$0.087  & \textbf{1.820}$\pm$0.078 \\
				\hline
				\multirow{2}{*}{gear}  & 2  & 3.311$\pm$0.046 & 3.150$\pm$0.037  & \textbf{3.430}$\pm$0.040 & 0.232$\pm$0.068 & \textbf{1.019}$\pm$0.048  & 0.590$\pm$0.043\\
				%\cline{2-5}
				& 3  & 3.538$\pm$0.048 & 3.347$\pm$0.045  & \textbf{3.721}$\pm$0.050 & 0.303$\pm$0.132 & \textbf{1.257}$\pm$0.085  & 1.020$\pm$0.064 \\
				%\cline{2-5}
				$n$=100 & 10  & 3.065$\pm$0.083 & 3.550$\pm$0.050  & \textbf{3.670}$\pm$0.067 & 0.312$\pm$0.232 & \textbf{1.566}$\pm$0.130  & 1.514$\pm$0.072 \\
				\hline
				\multirow{2}{*}{bedding}  & 2  & 3.406$\pm$0.080 & 3.374$\pm$0.088  & \textbf{3.620}$\pm$0.062 & 0.525$\pm$0.121 & 1.932$\pm$0.194  & \textbf{2.001}$\pm$0.080\\
				%\cline{2-5}
				& 3  & 3.648$\pm$0.106 & 3.564$\pm$0.083  & \textbf{3.876}$\pm$0.081 & 2.499$\pm$0.972 & 2.250$\pm$0.269  & \textbf{2.624}$\pm$0.066 \\
				%\cline{2-5}
				$n$=100 & 10  & 3.355$\pm$0.161 & 3.799$\pm$0.144  & \textbf{3.912}$\pm$0.082 & \textbf{3.919}$\pm$0.045 & 2.578$\pm$0.358  & {3.157}$\pm$0.091 \\
				\hline
				\multirow{2}{*}{apparel}  & 2  & 3.560$\pm$0.094 & 3.527$\pm$0.046  & \textbf{3.784}$\pm$0.059 & 0.268$\pm$0.109 & \textbf{1.552}$\pm$0.141  & 1.513$\pm$0.191 \\
				%\cline{2-5}
				& 3  & 3.878$\pm$0.092 & 3.755$\pm$0.062  & \textbf{4.140}$\pm$0.063 & 0.490$\pm$0.677 & 1.900$\pm$0.237  & \textbf{2.225}$\pm$0.136\\
				%\cline{2-5}
				$n$=100 & 10  & 3.751$\pm$0.087 & 4.084$\pm$0.075  & \textbf{4.425}$\pm$0.066 & 0.820$\pm$1.372 & 2.351$\pm$0.337  & \textbf{2.967}$\pm$0.150 \\
				\hline
				\multirow{2}{*}{bath}  & 2  & 2.957$\pm$0.087 & 3.024$\pm$0.032  & \textbf{3.198}$\pm$0.056 & 0.197$\pm$0.090 & \textbf{1.101}$\pm$0.083  & 0.795$\pm$0.078\\
				%\cline{2-5}
				& 3  & 3.062$\pm$0.085  & 3.195$\pm$0.058  & \textbf{3.448}$\pm$0.058 & 0.247$\pm$0.163 & \textbf{1.368}$\pm$0.134  & 1.269$\pm$0.059 \\
				%\cline{2-5}
				$n$=100 & 10  & 2.497$\pm$0.135 & 3.426$\pm$0.076  & \textbf{3.438}$\pm$0.089 & 0.327$\pm$0.312 & 1.711$\pm$0.183  & \textbf{1.742}$\pm$0.098 \\
				\hline
			\end{tabular}
		\end{center}
	\end{table}
}
